Exploring Failure Cases in Multimodal Reasoning About Physical Dynamics

In this paper, we present an exploration of LLMs' abilities to problem solve with physical reasoning in situated environments. We construct a simple simulated environment and demonstrate examples of where, in a zero-shot setting, both text and multimodal LLMs display atomic world knowledge about various objects but fail to compose this knowledge in correct solutions for an object manipulation and placement task. We also use BLIP, a vision-language model trained with more sophisticated cross-modal attention, to identify cases relevant to object physical properties that that model fails to ground. Finally, we present a procedure for discovering the relevant properties of objects in the environment and propose a method to distill this knowledge back into the LLM.

==> reviews.tex <==

----------------------- REVIEW 1 ---------------------
SUBMISSION: 3341
TITLE: Exploring Failure Cases in Multimodal Reasoning About Physical Dynamics
AUTHORS: Sadaf Ghaffari and Nikhil Krishnaswamy

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
The authors evaluate two LLM's (LLaMA2 and ChatGPT) and one language-vision model (LLaVA) in a simulated environment to evaluate their ability to arrange physical objects.  The three models are evaluated on the ability to move the correct objects and the resulting stability of the object configuration (e.g., that the objects do not topple over).  Additionally, another vision-language model, BLIP is also examined, but not empirically evaluated due to the fact it does not return textual output.  The results are largely negative: all four models suffer from the ability to correctly ground linguistic information to the associated correct objects.  The experiments are followed by a discussion on how to address these shortcomings.  They focus on adding in non-linguistic, non-visual information about objects (e.g., symmetries, affordances, does the object rotates, roll, etc.), exploiting LLM failure (i.e., executing LLM instructions until they become impossible).  The authors then propose a new framework to address these that deals with leveraging physical properties and exploration of the environment.

All in all this paper provides a solid set of well-presented experiments that dovetail nicely into a discussion of a future direction of research.  Further, the topic is highly relevant to the event (with the added focus on LLMs) and will be of interest to those in attendance.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 3341
TITLE: Exploring Failure Cases in Multimodal Reasoning About Physical Dynamics
AUTHORS: Sadaf Ghaffari and Nikhil Krishnaswamy

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
This paper explores some shortcomings of LLMs’ reasoning about physical dynamics, such as their inability to compose knowledge about individual objects into larger-scale reasoning. The paper provides a procedure to exploit failures in the zero-shot outputs of LLMs to investigate object interactions, and a method to feed learnings from these object interactions back into the LLM.

The topic of the paper is at the core of the symposium. The paper is well written and understandable. The approach of using failures to trigger simulation experiments and learning from them is intriguing and will lead to some good discussions at the workshop.

Some questions that the authors could address in the final version:

The experimental setup is very specific and to some extent artificial. Therefore, it is not clear how the results translate to actual real-world common-sense problems that involve physical dynamics. The results themselves are isolated, and it is unclear in what context they need/can be interpreted.

The section on Visual Grounding with Cross-Attention and BLIP offers some hypotheses as to why certain words (such as “round”, “flat”) guide the attention to certain objects in the image. This is useful. However, it remains unclear how much of the text structure (“the cylinder on its round side”) is relevant versus just the plain occurrence of words (“round”). This distinction seems important for the tasks at hand such as identifying objects and reasoning about the stability of object arrangements. Understanding the root of these deficiencies might shed light on how exactly knowledge bases like VoxML and the simulation environment can compensate.

Section Related Work, mathematical and logic problems. The first sentence is weird and unintelligible.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 3341
TITLE: Exploring Failure Cases in Multimodal Reasoning About Physical Dynamics
AUTHORS: Sadaf Ghaffari and Nikhil Krishnaswamy

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
The paper offers an insightful exploration into the limitations and potential of Large Language Models (LLMs) in understanding and reasoning within physical environments. The innovative approach of using LLMs' failures as a learning mechanism and the introduction of a methodology to reincorporate this learning into the models are commendable. The paper's focus on physical reasoning, object manipulation, and the use of BLIP for visual grounding align well with the symposium's theme. However, the authors might want to address the transfer into practice more clearly. The paper's novel perspective make it a valuable contribution to the symposium.
